An Investigation of Patch Porting Practices of the Linux Kernel Ecosystem

Open-source software is increasingly reused, complicating the process of patching to repair bugs. In the case of Linux, a distinct ecosystem has formed, with Linux mainline serving as the upstream, stable or long-term-support (LTS) systems forked from mainline, and Linux distributions, such as Ubuntu and Android, as downstreams forked from stable or LTS systems for end-user use. Ideally, when a patch is committed in the Linux upstream, it should not introduce new bugs and be ported to all the applicable downstream branches in a timely fashion. However, several concerns have been expressed in prior work about the responsiveness of patch porting in this Linux ecosystem. In this paper, we mine the software repositories to investigate a range of Linux distributions in combination with Linux stable and LTS, and find diverse patch porting strategies and competence levels that help explain the phenomenon. Furthermore, we show concretely using three metrics, i.e., patch delay, patch rate, and bug inheritance ratio, that different porting strategies have different tradeoffs. We find that hinting tags(e.g., Cc stable tags and fixes tags) are significantly important to the prompt patch porting, but it is noteworthy that a substantial portion of patches remain devoid of these indicative tags. Finally, we offer recommendations based on our analysis of the general patch flow, e.g., interactions among various stakeholders in the ecosystem and automatic generation of hinting tags, as well as tailored suggestions for specific porting strategies.

==> Strategies.tex <==
\section{root causes and analysis for patch delays}
\subsection{ Different porting strategies in different distros}
     
\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.5\textwidth]{figs/CVE_delay_distros_by_porting_strategies.png}
\end{center}
\vspace{-.2in}
 \caption{CVE patches delay with Linux mainline in different distros}
 \label{fig:CVE_delay_distros_by_porting_strategies}
 \vspace{-.2in}
\end{figure}

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.5\textwidth]{figs/CVE_delay_distros_by_porting_strategies_oneline.png}
\end{center}
\vspace{-.2in}
 \caption{CVE patches delay with Linux mainline in different distros}
 \label{fig:CVE_delay_distros_by_porting_strategies_oneline}
 \vspace{-.2in}
\end{figure}
\xingyu{combining all branches with the same porting strategies into oneline}
\xingyu{first only talk about following stable, lts and frequently rebase; arch only have little customization, so their delay with mainline is very short; but if stable branches does not have cve patches, then they will not be patched ,so this is the meaning of picking from mianline; divided into two parts: first is non-picking; second is only picking }
\xingyu{first, we know they are not from mainline, then we need to know their source(LTS or stable) and observer their base to see if they are following corresponding LTS or stable; giving general explaination of how we observer porting strategies then give examples like ubuntu }
\xingyu{frequently rebase is also following stable branches; but their tracking method is different from ubuntu-bionic, they rebase but not group-port and when stable branch reaches end-of-life, they rebase to another stable branch; delete how to track coloum}
\xingyu{more freuqently, shorter delay; but also methods of porting is also important; then introduce the framework, introduce porting strategies}
\xingyu{read more papers to know why each part is necessary; how each part motivate readers to continue to read}
\xingyu{think more to organize paper structures}
\xingyu{contact with prof.qian to discuss}

Linux distributions are operating systems which are based on the Linux kernel. Linux mainline keeps moving forward to incorporate new features and bug fixes. To stay up-to-date and keep bug-free, downstream Linux distributions need to propagate Linux patches from upstream. There are over 600 Linux distros and about 500 in active development according to \cite{Numofdistros} different Linux distributions; different Linux distributions are designed for different goals and maintained by different methods. Therefore, the way how they propagated Linux patches from Linux, called porting strategies, are also different. Porting strategies are vital to provide explanations for large patch delays discrepancies as it decides if and how a patch commit is propagated from upstream Linux to downstream distributions.

\xingyu{first, we know distros follow LTS or stable by observing commit logs; then when stable branches reaches end-of-life, what they do; except LTS and stable commits, are there commits from other sources}

To summarize porting strategies in Linux distributions, we need to  observe features of patch propagation behaviors for Linux distributions.   By extracting information in commit message, commit diff and commit authors, we can mine the patch propagation patterns between upstream and downstream. 

1)First, we realize that Linux distributions import continuous stream of commits in Linux stable and LTS branches by observing git commits logs of corresponding Linux distributions git repositories. It's common sense that Linux distributions pick and import patches from Linux mainline as Linux mainline incorporates the most and latest bug fixes. However, after observing information pertaining to git commits, we notice that distributions also follow Linux stable and LTS branches. In fact, Linux distributions pick individual mainline commit which is a fix to a specific security vulnerability, while they import almost all commits in a Linux LTS or stable release tag, such as "Linux v4.15.18". Besides, they follow Linux LTS or stable branches from the start to the end-of-life. 
% 1)First, we try to find their base point. We notice that some distributions, such as Ubuntu, are initially forked from a Linux mainline point and then keep moving forward on the top of the base; while others are based on a Linux stable or LTS kernel, such as KNOPPIX and Mageia, or based on a Linux distribution kernel, such as Linux mint, Scientific Linux and CentOS, and there are no modifications on the top of the base. 

2)Then, as the lifetime of Linux stable branches is only two or three months, we need to know the behaviors for distributions which follow Linux stable branches when Linux stable branch reaches end-of-life. We still mine such knowledge by observing git commits logs. There are different patch propagation behaviors. Ubuntu-bionic first track Linux 4.15 stable branch and then track neighbouring LTS branches, Linux 4.14 LTS and Linux 4.19 LTS, when Linux 4.15 reaches end-of-life. Ubuntu-trusty also tracks a Linux stable branch--Linux 3.13. Ubuntu maintainers, which are the Canonical Kernel Team(ckt), provide extended stable support for Linux 3.13 when it reaches end-of-life. Ubuntu-trusty continues to follow Linux 3.13-ckt. SLE15 also follows Linux stable branches and does not follow any Linux stable or LTS branches when Linux stable reaches end-of-life, and only pick commits from Linux mainline.
% 2)Then, we check the tracked branch, which is the source for commits which are propagated after the base. As mentioned in Section 2.1, Linux mainline introduces new features and patches, while Linux LTS and stable branches only accepts patches from Linux mainline. We notice that all of the observed Linux distributions do not follow Linux mainline directly, but to follow Linux stable or LTS branches. One reasonable guess is that Linux distributions do not pay attention to new features and only care bug fixes to make the base system less vulnerabilities. Distributions usually follow Linux LTS or stable branches which is forked from the same Linux mainline version. Their base is the same and should port the same patches. Linux LTS and stable maintainers already filter necessary bug fixes and adopt them if necessary. Following Linux LTS and stable branches can save lots of work and manual effort for Linux distributions. 

% 3)Next, we need to see their behaviors after Linux stable branches reach end-of-life. The lifetime of Linux LTS is six years, which exceeds the lifetime of most downstream Linux distributions, while the lifetime of Linux stable is only two or three months. There are different measures for distributions which follow stable branches. Some of them continue to track close Linux LTS branches, such as Ubuntu-bionic is based on Linux 4.15 stable branches and then follow Linux 4.14 and 4.19 LTS branches; some of them only pick commits from mainline, such as SLE; others change the base to the latest Linux stable branches. 

4)Finally, we also need to know if there are commits from other sources excepts commits from Linux stable and LTS branches. They may also pick commits from mainline, such as Oracle-uek branches and they may also write their own patches, such as sauce patches in Ubuntu.

The summary of porting strategies is in Figure~\ref{fig:strategies}. Linux distributions usually choose a Linux mainline version as its base to fork, while some distributions, taking Fedora and Arch as examples, they frequently rebase\xingyu{introduce the concept of git rebase} to the most recent Linux stable version. A release might be based on Linux 5.10.1 and propagate several important security patches from Linux mainline on the top of it; then it might be rebased to Linux 5.10.2 in a short period. Some distributions are only maintained by limited developers, such as KNOPPIX is mainly responsible by Klaus Knopper\cite{knopper}, so they directly use a Linux stable version as their kernel. Similarly, distributions, like Linux mint, directly use another Linux distribution kernel, which is Ubuntu for Linux mint. Some distributions fork from a Linux mainline version which has a corresponding LTS branch and then follow that LTS branches; at the same time, they also picks important security patches from Linux mainline. Ubuntu-focal is an example. Other distributions are similar and they also picks important security patches from Linux mainline, but their base is a Linux mainline version with a Linux stable branch and they continue to follow the Linux stable branch. However, the lifetime of Linux stable branch is only two or three months as mentioned in Section 2.1, when Linux stable branches reach end-of-life, some distributions continues to follow close LTS branches, such as Ubuntu-bionic, while some do not follow any LTS or stable branches and only pick from mainline. All in all, different distributions adopt different porting strategies.

\xingyu{find other more branches which do not have idle days to use them to show the influence of porting strategies on delay}
% \begin{figure}[hbt]
% \begin{center}
%   \includegraphics[width=0.6\textwidth]{figs/Strategies.png}
% \end{center}
% \vspace{-.2in}
%  \caption{porting strategies for distributions}
%  \label{fig:strategies}
%  \vspace{-.2in}
% \end{figure}

\begin{figure*}[t]
\begin{center}
\includegraphics[scale=0.3]{figs/strategies1.png}
\end{center}
\vspace{-.25in}
\caption{porting strategies for distributions}
\vspace{-.1in}
\label{fig:strategies}
\end{figure*}


% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=0.5\textwidth]{figs/group-ported_delay_ubuntus.png}
% \end{center}
% \vspace{-.2in}
%  \caption{delay in four Ubuntu branches}
%  \label{fig:group-ported_delay_ubuntus}
%  \vspace{-.2in}
% \end{figure}

Figure~\ref{fig:CVE_delay_distros_by_porting_strategies}, which clearly shows that frequently rebase > follow Linux LTS branches > follow Linux stable branches. \zheng{needs to clarify which are rebase/Follow LTS/Follow stable}



% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=0.5\textwidth]{figs/same_distro_same_strategies_sle.png}
% \end{center}
% \vspace{-.2in}
%  \caption{delay in SLE15-SP1,SLE15-SP2，SLE15-SP3}
%  \label{fig:same_distro_same_strategies_sle}
%  \vspace{-.2in}
% \end{figure}

\begin{figure}[t]
\begin{center}
  \includegraphics[width=0.5\textwidth]{figs/similar_base_different_stratgies.png}
\end{center}
\vspace{-.2in}
 \caption{delay in SLE15-SP1, UEK5 and Ubuntu-bionic}
 \label{fig:similar_base_different_stratgies}
 \vspace{-.2in}
\end{figure}
 

% If we eliminate the influence of different distributions, we get Figure~\ref{fig:group-ported_delay_ubuntus} 1) Ubuntu-trusty, Ubuntu-xenial and Ubuntu-focal are similar in delay and different from Ubuntu-bionic. These three adopt same porting strategies. Therefore, same porting strategies result in similar delay. Porting strategies can affect delay.
% 2) Ubuntu-trusty, Ubuntu-xenial and Ubuntu-focal are shorter in delay than Ubuntu-bionic. Ubuntu-bionic follows Linux stable branches and others three Ubuntu branches, follow Linux LTS branches. When stable branches reaches end-of-life, Ubuntu-bionic tracks two neighbouring branches, while it causes more commit filtering and adaptation work, resulting in longer delay.

% If we only care branches which are in the same distros and with the same porting strategies, we get Figure~\ref{fig:same_distro_same_strategies_sle_cve}: 1) They adopt same porting strategies and they are the same distributions, which means their maintainers and their time assignment are similar. So their are also similar in delay 2)Their delay are polylines but not smooth curve as lots of Linux stable minior version are group-ported at the same time(such as 4.12.1,4.12.2,4.12.3,4.12.4,4.12.5 are committed at the same time). Their delay is different from Ubuntu-bionic in previous figure. Even the same porting strategies, the method difference can cause different delay.

% From these two figures, porting strategies do influence the delay of different Linux distributions with upstream.

If we consider branches whose base is similar， such as in Figure~\ref{fig:similar_base_different_stratgies}, SLE-SP1 is based on Linux 4.14, Ubuntu-bionic is based on Linux 4.15 and Oracle-uek5 is based on Linux 4.14, they should patch similar bug fixes. \xingyu{here, we want to consider branches which should patch similar bugfixes and compare their delay, however, the conclusion from this figure is not clear and it may be discarded} 



If we combine different Linux distributions with same porting strategies into one line, we can get the
Figure~\ref{CVE_delay_distros_by_porting_strategies_oneline}. According to the figure, frequently rebasing porting strategies has the shortest delay. Distributions, like Fedora and Arch, are frequently rebased to a newer Linux stable version and only pick little patches from mainline to the base. Arch only add about three more commits after the base. As the customization is little, only chaning the base is easy. We keep checking the git commit status of fedora and arch git repositories to get the time on adaptation after rebasing for xxx days. And we found that there are only one or two days on picking less than thirty commits from Linux mainline and adapt them. The time is less on Arch, which is only about three commits and one day.  So it can be rebased to the latest Linux stable version quickly, resulting in short delay. On the other hand, the difference on the delay with mainline is not big as expected. Porting strategies does not affect delay much as three lines which represents different porting strategies are close. 
If the update and the work to port is as much as possible, the delay will be shorter.


\xingyu{the modification of figure 7}






% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=0.5\textwidth]{figs/same_distro_same_strategies_sle_cve.png}
% \end{center}
% \vspace{-.2in}
%  \caption{CVE patches delay with Linux mainline in different distros}
%  \label{fig:same_distro_same_strategies_sle_cve}
%  \vspace{-.2in}
% \end{figure}
    






% \textbf{3.1.2 Upstream first principle}
% \subsection{Upstream first principle}
% Almost all of distributions follow "Upstream first" principle. They want to keep close with upstream as much as possible. But one distributions -- Oracle Linux betrays it.



